Dirac Fermions in condensed matter and beyond

This review aims at a theoretical discussion of Dirac points in two-dimensional systems. Whereas Dirac points and Dirac fermions are prominent low-energy electrons in graphene (two-dimensional graphite), research on Dirac fermions in low-energy physics has spread beyond condensed-matter systems. In these alternative systems, a large versatility in the manipulation of the relevant band parameters can be achieved. This allows for a systematic study of the motion and different possible fusions of Dirac points, which are beyond the physical limits of graphene. We introduce the basic properties of Dirac fermions and the motion of Dirac points here and aim at a topological classification of these motions. The theoretical concepts are illustrated in particular model systems.

==> bourbaphydefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin of definition file AHPEFS.TEX                      %
% (c) Stephan Ammann, for Birkhaeuser, Dec 1999            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AHPDEFS.tex -- is red in by each header file             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\font\fxtit=cmssbx10 % For the new logo

\newcount\fpage\newcount\npage\newcount\lpage
\fpage=\fipage\npage=\nrpage
\lpage=\fpage\advance\lpage by\npage\advance\lpage by-1

\def\xrule{\vrule width2.25pt}
\def\yrule{\hrule height.5pt}
\def\yrulefill{\leaders\yrule\hfill}
\def\strutx{\vrule height8.5pt width0pt depth0pt}
\def\struty{\vrule depth3.5pt width0pt}
\def\strutz{\vrule height10.2pt width0pt}

\def\boxl{\vbox{\halign{##\hfil\cr
S{\'e}minaire Poincar{\'e} \volnr\ (\centnr\yearnr)
\the\fpage\ -- \the\lpage\cr
%\struty \copyright\ Birkh{\"a}user Verlag, Basel,
%\centnr\yearnr\cr
%1424-0637/\yearnr/\issuenr0\fipage-\the\npage\ \ %
%\$\,1.50$+$0.20/0\cr
}}}


\def\boxr{\vbox{\offinterlineskip
\halign{##\hfil\hskip1mm&##\hfil\cr
\noalign{\vskip.8mm}
\multispan2{\yrulefill}\cr
\xrule\strutz\struty
&\fxtit S{\'e}minaire Poincar{\'e}\cr
%\xrule\strutx&%
%\vbox to0pt{%
%\vbox to0pt{\vss\hbox{\fxtit and Applications NoDEA}}\vss}\cr
}}}

\def\titlebox{\vbox to0pt{\hsize=150mm\footnotesize\vss
\hbox to\hsize{\boxl\hfil\boxr}}}


\def\ps@myheadings{
\let\@mkboth\markboth
\def\@oddhead{\footnotesize \rm Vol. \volnr, \centnr\yearnr
\hspace{6mm}\titletxt\hfil\thepage}%
\def\@oddfoot{} % % centered page number
\def\@evenhead{\footnotesize \thepage \hfil
\authortxt\hspace{6mm}S{\'e}minaire Poincar{\'e}}%
\def\@evenfoot{}%       % centered page number
}

\def\ps@plain{
\let\@mkboth\markboth
\def\@oddhead{%
\titlebox}%
\def\@oddfoot{}%      % centered page number
\def\@evenhead{}%
\def\@evenfoot{}%     % centered page number
}

\ps@myheadings              % 'myheading' page style
\pagenumbering{arabic}      % Arabic page numbers
\onecolumn                  % Single-column.

\setcounter{page}{\fpage}

\textwidth=150mm
\textheight=230mm
\parindent=8mm
\evensidemargin=0pt
\oddsidemargin=0pt
\topmargin=0pt
\frenchspacing

\newcommand{\pdpg}{\postdisplaypenalty=-2000}
%% Used to force a page-break after a displayed equation

\let\dst=\displaystyle
\let\scr=\scriptstyle

\def\bfdefault{b}

\def\Rec{Received\ }
\def\Rev{Revised\ }

\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of AHPDEFS.TEX                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of definition file

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: t
%%% TeX-master: t
%%% TeX-master: t
%%% End: 

